Few-Shot Anaphora Resolution in Scientific Protocols via Mixtures of In-Context Experts

Anaphora resolution is an important task for information extraction across a range of languages, text genres, and domains, motivating the need for methods that do not require large annotated datasets. In-context learning has emerged as a promising approach, yet there are a number of challenges in applying in-context learning to resolve anaphora. For example, encoding a single in-context demonstration that consists of: an anaphor, a paragraph-length context, and a list of corresponding antecedents, requires conditioning a language model on a long sequence of tokens, limiting the number of demonstrations per prompt. In this paper, we present MICE (Mixtures of In-Context Experts), which we demonstrate is effective for few-shot anaphora resolution in scientific protocols (Tamari et al., 2021). Given only a handful of training examples, MICE combines the predictions of hundreds of in-context experts, yielding a 30% increase in F1 score over a competitive prompt retrieval baseline. Furthermore, we show MICE can be used to train compact student models without sacrificing performance. As far as we are aware, this is the first work to present experimental results demonstrating the effectiveness of in-context learning on the task of few-shot anaphora resolution in scientific protocols.

==> commands.tex <==
\newcommand\mice{\textsc{Mice}}
\newcommand\micesamp{\textsc{Mice-Sampling}}
\newcommand\singlerand{\textsc{SingleRandom}}
% \newcommand\singlesim{\textsc{SingleSimilar}}
\newcommand\singlesim{\textsc{Kate}}
% \newcommand\kate{\textsc{Kate}}
\newcommand\kate{\textsc{Kate}}
\newcommand\product{\textsc{Product}}
\newcommand\etoe{E2E}
\newcommand\knowdist{Knowledge Distill.}

\newcommand\chemuref{\textsc{ChEMU-Ref}}
\newcommand\procbert{\textsc{ProcBERT}}

\newcommand\fscore{\text{F$_1$}}

==> old/sections/0_abstract.tex <==
Split-antecedent resolution-- resolving plural mentions to multiple previous antecedents-- plays an important role in anaphora resolution and information extraction applications. However, this task is less studied than their coreference resolution counterpart, mostly due to the lack of large-scale annotated resources available. At the same time, research on learning from limited training data (\textit{i.e.} few-shot learning) has received increasing attention, thanks to the creative applications of large pre-trained language models. In this work, we study whether \textit{in-context learning}, a particular paradigm of few-shot learning, can be effectively applied to split-antecedent resolution, where few-shot is a natural setting given the limited data available. Our results and analysis show that simple extensions of in-context learning can achieve significant performance gains in difficult tasks and domains beyond popular NLP benchmarks. \Max{This punchline needs something a bit stronger. Highlight our work is pioneering for \textit{span-based} tasks?}

==> old/sections/1_intro.tex <==

Split-antecedent resolution systems determine how to link anaphors to their corresponding antecedents in a given text. \footnote{Also known as multi-antecedent resolution \cite{vala-etal-2016-antecedents}} The task plays an important role in the difficult task of anaphora resolution, as well as information extraction for procedural and scientific texts (Figure \ref{fig:task_examples}). Existing work for this task followed coreferece resolution literature and employed neural ranking models that often needs to be trained on large amount of data in order to achieve high performance \cite{lee-etal-2017-end, joshi-etal-2020-spanbert, wu-etal-2020-corefqa}. Since annotated data are limited, current systems use data augmentation \cite{yu-etal-2020-free} or train on single-antecedent data \cite{yu-etal-2021-stay} to improve performance. Nonetheless, there are still ample room for improvement. 

\begin{comment}
\begin{figure}[t]
    \centering
    \includegraphics[scale=0.32]{figures/task_examples.pdf}
    \caption{Task Examples Placeholder. Final figures should have 1) general ARRAU 2) chemical procedures, something with "the mixture" (3) cooking recipes}
    \label{fig:task_examples}
\end{figure}
\end{comment}

At the same time, research in few-shot learning is making substantial progress \cite{schick-schutze-2021-exploiting, gao-etal-2021-making, ram-etal-2021-shot}, driven mainly by creative applications of large pre-trained language models \cite{gpt3, bert, t5, petroni-etal-2019-language}. This line of research gives rise to \textit{in-context learning}-- a paradigm where the model is able to make accurate predictions by conditioning on a few in-context examples (input-label pairs) \cite{liu2021makes, Rubin2021LearningTR, metaICL, minWhyInContext}. Most of these work are evaluated on popular text classification and question-answering benchmarks \maxle{cite some benchmarks}. 
\Max{Need to fact-check the above paragraphs/literature reviewed more carefully. At least there is Schick and Schutze with PET for text generations}

In this work, we are asking whether existing few-shot techniques can be effectively applied to the difficult task of split-antecedent resolution. This task serves as an interesting venue to evaluate existing few-shot techniques, given limited annotated data \maxle{Use a lot of "limited annotated data"-- find ways to utilize "under-resourced task"}. We focus on applying and extending in-context learning paradigm to fit our task specifications. Since the task is challenging even given full gold anaphors and gold mentions \cite{yu-etal-2020-free}, we assume gold anaphors are given.
\Max{TODO. Add more our approach and results here. Thesis and contribution of this work: (1) simple extension of in-context learning to improve split-antecedent anaphor (2) analysis and datasets}

==> old/sections/2_task.tex <==
\paragraph{Task Definition} We follow previous work in defining the split-antecedent resolution task \cite{vala-etal-2016-antecedents, yu-etal-2020-free}. In the most general setting, given a document-level text $D$, for each mention $m$ in the set of identified mentions $\mathcal{M}$, the task is to predict the subset $\mathcal{Y}_m \subseteq \mathcal{M}$ containing mentions that are antecedents to $m$. If $\mathcal{Y}_m = \emptyset$, then $m$ is non-anaphoric.
Split-antecedent resolution involves two subtasks: anaphor detection where the system identifies the mentions that are anaphoric, and antecedent resolution where the system predicts which of the previous antecedents map to each identified anaphor. \footnote{Some work adds a subtask at the beginning: mention detection to identify all the relevant mentions in the text} Given the complexity of the task, previous work often focused on antecedent resolution subtask and assumed gold mentions and/or gold anaphors \cite{vala-etal-2016-antecedents, yu-etal-2020-free}, defaulting mention/anaphoric detection to an off-the-self mention detector. Several recent work proposed joint modelling of the two subtasks \cite{yu-etal-2021-stay, fang-etal-2021-chemu}.

In this study, we adopt the pipeline approach without assuming access to gold mentions or anaphors.  Our anaphor detection system takes in document $D$ and output a list of predicted anaphors $\mathcal{A}$. The anaphora resolution step, which is also the focus of this study, takes in each anaphor $a \in \mathcal{A}$ along with the original document and predicts a set of antecedents $\mathcal{Y}_a$. 

\paragraph{Anaphor Detection} For anaphor detection step, we develop a simple rule-based system using string matching heuristics (Appendix \ref{app:anaphor_detection}). Given that the majority of anaphors in our dataset are common plural mentions(\textit{e.g.} \textit{the solution, the mixture, the resulting solution}, etc.), our system can effectively identify these anaphoric mentions, achieving high F1 score when evaluated on the ChEMU-Ref test set (Table \ref{tab:anaphor_detection}).

\begin{table}[!t]
\centering
\begin{tabular}{lccc}
\hline
 & P & R & F1 \\
\hline
ChEMU-Ref & 97.6 & 95.7 & 96.6 \\
%RecipeRef & & & \\
%ARRAU & 74.1 & 83.8 & 78.4 \\
\hline
\end{tabular}
\caption{Results of our rule-based anaphor identification system.
\Max{This table can be moved to Appendix if we need more space}
}
\label{tab:anaphor_detection}
\end{table}

\paragraph{Datasets} 
% The most widely used dataset to evaluate split-antecedent resolution is the ARRAU corpus \cite{ARRAU}, which annotated a wide-range of anaphoric information (split-antecedent plurals; discourse deixis; and bridging references). Following previous work, we use the RST portion (news text) of ARRAU, and only focus on the split-antecedent plurals annotation. In addition, to ARRAU, we also evaluate our approach on the ChEMU-Ref \cite{fang-etal-2021-chemu} and RecipeRef datasets, which contain anaphoric information in chemical procedures and cooking recipes, respectively. An advantage of using these datasets is that split-antecedent anaphors exist in abundance in procedural texts, thus serving as an ideal domain to study this problem. Relevant dataset statistics are shown in Table \ref{tab:datasets} \Max{Need to justify not using ARRAU if we cite ARRAU-related work}.
% \begin{table}[!t]
% \centering
% \begin{tabular}{lccc}
% \hline
%  & ChEMU-Ref & RecipeRef & ARRAU \\
% \hline
% Doc. & & &  \\
% Anaphor & & &  \\
% Ante. & & &  \\
% Sentence & & &  \\
% Token & & &  \\
% \hline
% \end{tabular}
% \caption{Statistics of the ChEMU-Ref dataset used in this study}
% \label{tab:datasets}
% \end{table}
To evaluate our approach, we mainly use ChEMU-Ref, a corpus of chemical procedures for coreference and anaphora resolution \cite{fang-etal-2021-chemu}. While the dataset is annotated with fine-grained, chemistry-specific annotations, we are interested in exploring the coarser "contained" relation between mentions. Thus, we pre-process the data by collapsing the fine-grained relations into a single \texttt{Contained} relation. In addition, we perform transitive closure between anaphoric and non-anaphoric mentions. For example, if "the solution" contains "water" and "sodium", and "the mixture" contains "the solution", then "the mixture" contains "water" and "sodium".
\Max{TODO: Revisit to make this clearer. Maybe helpful with a Figure 1 in the Introduction?}

\paragraph{Few-shot Setting} In our study, we define each example to consist of a document $D$ and an anaphor $a$, with gold antecedents set $\mathcal{Y}_a$. The few-shot training dataset $\mathcal{D}_{train}$ then contains $K$ examples. We experiment with values of $K \in \{4, 8, 16, 32, 64\}$. Following recommendations from \cite{Perez2021TrueFL}, we limit the size of the development set $\mathcal{D}_{dev}$ to 64 examples. This is faster than using K-fold cross-validation while still within the rough estimate of training examples for few-shot learning.\footnote{The total number of training examples $|\Dc_{train}| + |\Dc_{dev}|$ never exceeds 128.} Details of how we sample $\mathcal{D}_{train}$ and $\mathcal{D}_{dev}$ can be found in the Appendix \ref{app:data}.\ar{Does Perez et. al. use 64 examples for a dev set?  From looking through the paper, it sounds like the are doing K-fold cross-validation, which is different/slower than what we are doing.}\maxle{@AR: while \cite{Perez2021TrueFL} experimented with K-fold cross-validation, they did recommend other approaches in their conclusion, such as including the number of dev set in the total of few-shot training examples}

\begin{table}[!t]
\centering
\begin{tabular}{lccc}
\hline
& Train & Dev. & Test \\
\hline 
Documents &  & & \\
Anaphors & & & \\
Antecedents & & & \\
Sentences & & & \\
Tokens & & & \\
\hline
\end{tabular}
\caption{Statistics of the ChEMU-Ref dataset used in this study. TODO: Need to figure out what makes sense to report for train
\Max{This table can be moved to Appendix if we need more space}
}
\label{tab:datasets}
\end{table}

==> old/sections/3_method.tex <==
We propose to use in-context learning as a possible approach for the anaphora resolution step. For in-context learning to be possible, we first need to reformulate the task as text generation (Section \ref{sec:in_context_single}). We then propose Mixture of In-context Experts as an effective ways to combine predictions to multiple prompts (Section \ref{sec:in_context_mice}) and its sampling approximation (Section \ref{sec:in_context_sampling}). Finally, we evaluate our proposed methods in Section \ref{sec:in_context_eval}.
\Max{TODO: last sentence explicitly states the results eg "empirical evaluation shows that..."}

\subsection{In-context Learning}
\label{sec:in_context_single}

In-context learning requires an input \textit{prompt} into an autoregressive language model (e.g. GPT-3) and outputs a sequence of tokens. Our prompt has two main elements: (1)  the test input $(D_{test}, a_{test})$ and (2) the set of corresponding \textit{in-context demonstrations}. Important considerations for prompt design includes prompt template as well as the number, the retrieval, and the ordering of in-context demonstrations

\paragraph{Prompt Template} Given an input $(D, a)$, prompt template function $\Tc$ converts it into natural language text $x = \Tc(D, a)$.\footnote{From now on we will refer to $x$ as the test input, instead of the more cumbersome notation $\Tc(D, a)$} For in-context demonstrations, we also include the gold antecedents in the text ($x = \Tc(D, a, \mathcal{Y}_a)$) by linearizing the gold antecedents using their surface forms, separated by a separator token. Previous work establishes that different formats can significantly impact the in-context learning performance \cite{schick-schutze-2021-just, gao-etal-2021-making}. In this work, we mainly use QA-style format (Figure \ref{fig:approach}). We experiment with other formats and TODO conclusion (Section \ref{app:prompt_hyperparameters}). 

\paragraph{Number of In-context Demonstrations} Each test input corresponds to $k$ in-context demonstrations.\footnote{This $k$ is often referred as $k$-shot, which is different from $K = |\Dc_{train}|$} The value of $k$ varies between different settings, depending on the max context size of the language models and the length of the demonstrations. Previous work often experimented on tasks with short sentence-level input (e.g. text classifications), therefore the LM encoder is able to fit up to 32 examples \cite{gpt3}. In contrast, our setting requires longer, document-level context, thus limiting the amount of demonstrations that can be encoded in the LM, even given the max context length available of 2048. As a result, we default $k=2$ in all our experiments. \ar{At some point we need to explain that we only use 2 in-context examples per prompt and justify this choice.  E.g. is this because adding more than 2 examples doesn't improve performance?  Or because they don't fit in the maximum length of the encoder?  Or both?}
\Max{@AR: Choice of 2 in-context examples is mainly due to exceeding max context length. We can also experiment with different values of $k$ (eg 0-3), + see how much of the examples fit in the context and not} 

\paragraph{Retrieval of In-context Demonstrations} The choice of which demonstrations from $\mathcal{D}_{train}$ to include with a given a test input is the subject on ongoing research \cite{liu2021makes, Rubin2021LearningTR}. In this work, we experimented with random and KNN-based retrieval methods. 

\paragraph{Ordering of In-context Demonstrations} \citet{Zhao2021Calibrate} and \citet{Lu2022Fantastically} show that the order (\textit{i.e.} permutation) of the prompt examples can significantly impact the performance of in-context learner. This effect is less pronounced in our setting, given the limited number of demonstrations in each prompt ($k=2$).

\paragraph{Contextual Calibration} Previous work \citep{Zhao2021Calibrate, holtzman-etal-2021-surface} has shown that prompted LMs can be biased towards specific labels, regardless of the test input. As a result, different calibration procedures to help alleviate these biases have been proposed \cite{Zhao2021Calibrate, holtzman-etal-2021-surface} and successfully applied to text classification \cite{Min2021NoisyCL, Lang2022Cotraining} and relation extraction \cite{gutierrez2022thinking} tasks. Following previous work, we adopted the calibration procedure for generation tasks described in Section 5 of \citet{Zhao2021Calibrate}, also referencing their code.\footnote{\url{https://github.com/tonyzhaozh/few-shot-learning}} Specifically, we compute calibration parameters using the output probabilities of the content-free prompt (\textit{e.g.} prompt with "N/A" test input), and use these parameters to update output probabilities when prompted with test inputs. However, we found that applying this calibration procedure consistently reduces performance.  When prompted with content-free inputs, the language model typically generates bias-free answers (including "N/A", a blank line, or "Null").  This suggests there is no significant bias towards specific context-free answers the case of split-antecedent anaphora resolution, making calibration unnecessary for our task and prompt design.
%The language models prompted with in-context demonstrations do not suffer from significant biases, 
%, as identified in \cite{Zhao2021Calibrate} and thus existing calibration methods are unsuitable for this task.

% \subsection{Combination of In-context Learners}
% \label{sec:ensemble_in_context}

% We describe a simple method of ensembling the in-context learners that can effectively outperforms various baselines for few-shot split-antecedent. While various single in-context learners failed for this setting, an ensemble of such learners can reduce the variance, each with either randomly or similarity-based sampled prompts. 
% The general algorithm is shown in Figure \ref{fig:ensemble_approach}

% \paragraph{Prompts Generation} We generate a fixed number of $t$ prompts for our ensemble, with the number of prompts $t \leq k^2$, since we have two examples in each prompt (Section TODO). Note that the examples in a prompt can have arbitrary ordering. We experiment with two prompt generation methods:
% \begin{itemize}[noitemsep]
%     \item Random: Given a total number of possible prompts $k^2$ from the training set $\mathcal{D}_{train}$ of size $k$, we randomly sample $t$ prompts without replacement.
%     \item Similar: Given test example $X_{test}$, we first find the top-$\sqrt{t}$ examples (after converting with template function $\mathcal{T}(X)$ most similar to $\mathcal{T}(X_{test})$. For example, if $t=100$, we first find top-10 most similar example to the test example, then we construct the prompts by using all those 10 examples in a pair-wise manner. For example retrieval, we use off-the-shelf retrieval (Section TODO).  \ar{If I were reviewing this paper, I think I would question how interesting/significant the conclusion is that "Random" works better than "Similar".  I *think* the only reason to select a subset of the training examples based on similarity is if they can't all be encoded into the prompt.  But I guess this is one of the main advantages of our prompt combination method - it can effectively encode all of these longer in-context demonstrations.}
% \end{itemize}

% \paragraph{Combining Predicted Antecedents} The LM will generate $t$ sequences $\yb_1, ..., \yb_t$ from the $t$ input prompts. We first de-linearize the sequences into $t$ predicted antecedent sets $\hat{E}_1,...,\hat{E}_t$, from which we construct a unique predicted mention set $\mathcal{M}_{X_{test}}$. We then use information from the different generations, via count-based or probabilistic methods, to construct the final predicted antecedent set (Section \ref{sec:combination_methods})

\subsection{Mixture of In-context Experts (MICE)}
\label{sec:in_context_mice}

\begin{figure*}[!t]
    \centering
    % \includegraphics[width=\textwidth]{figures/approach-crop.pdf}
    \includegraphics[width=\textwidth]{figures/approach.pdf}
    \caption{TODO}
    \label{fig:approach}
\end{figure*}

While in-context learning with large language models has achieved surprisingly good performance when learning from few examples, the performance can vary significantly depending on different prompt orderings.  Furthermore, these methods struggle to handle longer demonstrations and larger numbers of examples.
%that can be encoded is limited by the sequence length restrictions found in many large-scale models.

To address these challenges we propose Mixtures of In-Context Experts (MICE), which effectively combine larger numbers of in-context demonstrations.  Each prompt encodes a pair of training examples in context, so that the total number of prompts can be be up to $K^2$.

Each prompt is modeled as a latent variable $z$.  After encoding the prompt, together with a candidate test input $x$, the language model (e.g. GPT-J) can be used to calculate the probability that antecedent $i$ will be generated given prompt $z$ and input $x$, $P(y_i=1|z,x)$.  To combine probabilities across the $k^2$ in-context experts, we employ a mixture model:
\begin{equation}
P(y_i=1|z,x) = \sum_z P(y_i=1|z,x) P(z|x)
\label{eq:mice}
\end{equation}
where $y^*_i$ is a one-hot vector representing the $i$th antecedent in the set of candidates, $\mathcal{Y}$.  $P(z|x)$ is computed based on a measure of similarity between $x$ and the two training examples $u, v$ encoded in $z$:
\[
P(z|x) \propto \exp{(s_{x,u} + s_{x,v})}
\]
\Max{How to compute similarity scores $s_{x,u}, s_{x,v}$ TODO}

\ar{TODO: Need to make this part clearer}
$P(y=i|z,x)$ in equation \ref{eq:mice} is the probability that the LM predicts the $i$th antecedent for an input anaphor, $x$. Practically, we estimate $P(y_i|z,x)$ using the probability assigned by the LM to the first token in $y_i$ at the first position of every $y_j \in \mathcal{Y}(z,x)$. \footnote{Similar to \citet{Zhao2021Calibrate}, we found that after generating the first token in the span, subsequent tokens are deterministic.} $P(y_i|z,x)$ is then equivalent to the max of all $P(y_j = y_i|z, x)$.
\[
P(y_i|z,x) = \max_j P(y_j = y_i|z, x)
\]

As we will show shortly, the mixture of in-context experts is a very effective way to combine the strengths of individual antecedent prediction prompts.  However, this method requires storing logits for all tokens in the vocabulary so that $P(y_i|z,x)$ can be computed for all candidate antecedents, once they are generated, which is slow and require significant storage for mixtures with a large number of prompts.  In the next section we describe a more efficient solution that we found to give similar results as described in \S \ref{sec:experiment}.

\subsection{Simple and Efficient Approximation via Sampling}
\label{sec:in_context_sampling}
To address these challenges, we found that a simple sampling-based approach that approximates MICE achieves comparable results.  Rather than summing over all candidate antecedents, we approximate $P(\mathbf{y}|x)$ through sampling:
\begin{eqnarray*}
P(y_i=1|x) & = & \sum_z P(y_i=1|z,x) P(z|x) \\
    & \approx & \sum_z \mathbbm{1}[i \in \mathcal{Y}(z,x)] P(z|x)
\label{eq:sampling}
\end{eqnarray*}
\maxle{Would we also want to summarize this equation in text?}
where $\mathcal{Y}(z,x)$ is the set of antecedents generated by the LM when prompted with in-context demonstrations $z$ test input $x$.  Estimating $P(y_i=1|z,x)$ by monte-carlo sampling avoids the need to compute LM probabilities for all possible antecedents given each prompt, making the mixture of in-context experts simpler to implement and more efficient.  In \S \ref{sec:experiment}, we show empirically that there is no significant loss in performance when approximating the LM probabilities through sampling.

\begin{comment}
Given the noisy predicted mention set $\hat{E}$ aggregated from the different LM generations, we want to output mentions that the ensemble of in-context learners are most confident in. We do some by computing the predicted mention probability $P(\mh \mid Z_1,...,Z_t)$, for all $\mh \in \hat{E}$, then taking the predicted mentions with high probability. This section describes three different models to compute $P(\mh \mid Z_1,...,Z_t)$ that utilize different information from the LM generations. 

\paragraph{Count-based Model} This model computes the mention $\mh$ probability by simply aggregating the count of $\mh$ in the predicted antecedent sets, divided by the total count of all predicted mentions 
\begin{equation}
    % P(\mh) = \frac{\text{count}(\mh)}{\text{total count}}
    P(\mh \mid Z_1,..., Z_t) &= \frac{\sum\limits_{i=1}^t \sum\limits_{m' \in \hat{E}_t} \mathbb{1}(m' = \mh)}{\sum\limits_{m \in \mathcal{M}_{test}}\sum\limits_{i=1}^t \sum\limits_{m' \in \hat{E}_t} \mathbb{1}(m' = m)}
\end{equation}
\maxle{Lots of (unnecessary?) symbols here. TODO simplify. We can formalize this eg using $\mathbb{1}$ function}

\paragraph{Noisy-OR Model} The count-based model does not take into account the generation probability from the language model. To incorporate this information, we experiment with the \textit{Noisy-Or model}: 

\begin{equation}
    P(\mh \mid Z_1,..., Z_t) = 1 - \prod_{i=1}^t P(\mh = 0 \mid Z_i)
\end{equation}

where $P(\mh=0 \mid Z_i)$ is the LM probability of the of $\mh$ if $\mh$ is \textit{not predicted} by the LM conditioned on prompt $Z_i$. $P(\mh=0 \mid Z_i)$ is computed as follows:
\begin{equation}
    P(\mh = 0 \mid Z_i) = 1 - \max_{0 \leq j \leq |\hat{E}_i|} P(\mh_j \mid Z_i)
\end{equation}

where $P(\mh_j \mid Z_i)$ is the probability that the LM predicts $\mh$ at position $j$ within the predicted mentions. Practically, we estimate $P(\mh_j \mid Z_i)$ by using the probability that the LM generates the first token in $\mh$ at the first position of every predicted mentions indexed $j$ in $\hat{E}_i$. \footnote{Similar to \cite{Zhao2021Calibrate}, we found that after generating the first token in the span, subsequent tokens are deterministic.} $P(\mh \mid Z_i)$ is then equivalent to the max of all $P(\mh_j \mid Z_i)$.

\paragraph{Mixture Model} The previous two models explicitly conditioned on the prompts $Z_1, ..., Z_t$. In the mixture model, we directly model $P(\mh \mid X_{test})$ by treating $Z_1, ..., Z_t$ as latent variables: 

\begin{equation}
    P(\mh \mid X_{test}) = \sum_{i=1}^t P(\mh \mid Z_i, X_{test})P(Z_i \mid X_{test})
\end{equation}
Similar to the Noisy-OR model, $P(\mh \mid Z_i, X_{test})$ is the LM probability of the (first token) of $\mh$, conditioned on prompt $Z_i$. In contrast, the distribution of $P(Z_i \mid X_{test})$ depends on the prompt generation process: random generation will give uniform distribution $P(Z_i \mid X_{test}) = 1/t$, whereas similar prompt generation, $P(Z_i \mid X_{test})$ is estimated using the dot product between $s_{test, j}, s_{test,k}$:
$$P(Z_i\mid X_{test}) \propto \exp{(s_{test,j} \cdot s_{test,k})}$$
where $s_{test, j}, s_{test,k}$ are the similarity scores between $X_{test}$ and the two in-context examples $X_j, X_k$ in $Z_i$, respectively. 
\end{comment}

\subsection{Empirical Evaluation of Prompt Combination Methods}
\label{sec:in_context_eval}

\begin{table}[!t]
\centering
\begin{tabular}{lcc}
\hline
& \textbf{$K$=32} & \textbf{$K$=64} \\
\hline
Random Single & 37.6_{2.8} & 39.6_{3.7} \\
% Random Single Calibrated & 36.4 & & \\
Similar Single & 40.0_{7.8} & 42.7_{4.2} \\
% Similar Single Calibrated & 34.2 & & \\
\hline
Sampling & 62.7_{3.5} & 63.7_{3.2} \\
%Similar Count-based & 65.7 & & \\
% Noisy-OR & \textbf{63.1}_{2.7} & \textbf{63.8}_{2.7} \\
%Similar Noisy-OR & 64.5 & & \\
% Mixture-Model w/ uniform & 62.3_{2.5} & 62.3_{2.7} \\
MICE & 62.3_{2.5} & 62.4_{2.6} \\
%Similar Mixture-Model & 66.3 & & \\
\hline
\end{tabular}
\caption{We investigate the effects of different prompt generation and combination methods, showing the F1 results for $K=32, 64$ on dev set. The number of prompts used for combination-based models is 256.  Means and standard deviations are reported over five trials with randomly sampled training examples.}
\label{tab:combination_methods}
\end{table}

We empirically evaluate different combination methods mentioned in Section \ref{sec:in_context_mice} (MICE) and Section \ref{sec:in_context_sampling} (Sampling). We also compare these multi-prompted models with their single-prompted counterparts: Random Single where we randomly sample two in-context demonstrations for each test input, and Similar Single where we encode two most similar examples to the test input. Results are shown in Table \ref{tab:combination_methods}. We observe that multi-prompted models significantly outperformed single-prompted models as well as reduced the variance between trials. Among the multi-prompted models, Sampling achieved higher F1 than MICE, but both models are within standard deviations of each other. 

\paragraph{Span-based Verbalizers}\maxle{TODO Rethink this section}
 In preliminary experiments, we found that the predicted mentions suffer from \textit{surface-form competition} problem \cite{holtzman-etal-2021-surface}, where the LM can generate spans not observed in the context, but means the same concept (\textit{e.g.} \textit{"water (50 ml)"} vs. \textit{"50 ml of water"}). To address this, we extend the \textit{verbalizer} concept \cite{schick-schutze-2021-just} from text classification to span-based tasks. Specifically, we propose the span-based verbalizer function $v$ that maps the gold span to its equivalent, paraphrased spans. For example, $v(\textit{"water (50 ml)"}) = \{\textit{"water (50 ml)", "50 ml of water", "water"}\}$. Each combination method can then aggregate the probabilities from these spans (Figure \ref{fig:ensemble_approach}. The verbalizer function $v$ is constructed using heuristic rules (see Appendix \ref{app:span_based_verbalizer}). Note that these probabilistic aggregation of generated answers has been applied in various forms in the in-context learning literature, most prominently in text classification tasks \cite{Lang2022Cotraining, holtzman-etal-2021-surface}. 

\section{Knowledge Distillation (Self-training)}
Large language models like GPT-3 \citep{gpt3} show great few-shot capacities with in-context learning. However, it is hard to deploy them in real-life applications due to their prohibitive inference cost. To address this bottleneck, we perform knowledge distillation, where we distill few-shot capacities from a large prompted teacher model to a smaller inference-efficient student model. Specifically, given $k$ labeled examples, we build an ensemble model by aggregating $t$ prompted in-context learners via the count-based method. We use this ensemble model to generate pseudo labels for 500 or 1000 unlabeled examples. Then we train a smaller BERT-based student model like \citet{fang-etal-2021-chemu} on the pseudo labels to see whether this distillation procedure produces a smaller performant model, which preserves the knowledge in the teacher model.

\begin{figure*}
  \includegraphics[width=\textwidth]{figures/knowledge_distill-cropped.pdf}
  \caption{Overview of the knowledge distillation method.}
  \label{fig:knowledge_distill}
\end{figure*}

\begin{table*}[th!]
\small
\begin{center}
% \scalebox{0.6}{
\setlength{\tabcolsep}{3pt}%Tighter
% \resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccc}
\toprule 
\multirow{3}{*}[-0.3em]{\textbf{Datasets}} & \multicolumn{4}{c}{\textbf{$k$=32}} & \multicolumn{4}{c}{\textbf{$k$=64}} \\
\cmidrule(l){2-5} \cmidrule(l){6-9} 
 & ensemble & gold-32 & pseudo-500 & pseudo-1000 & ensemble & gold-64 & pseudo-500 & pseudo-1000 \\ \midrule
\textsc{ChEMU-Ref} & 61.5 & 47.5 & 53.7 &  \\
\textsc{RecipeRef} &  &  &  &  \\
% \textsc{ARRAU}     &  &  &  &  \\
 \bottomrule
\end{tabular}
% }
% }
\end{center}
\caption{\label{tab:knowledge_distill} Test set $F_1$ of knowledge distillation experiments on three datasets, where we train the BERT-based baseline under two settings: 1) $k$ examples with gold labels; 2) 500 or 1000 examples with pseudo labels generated by the $k$-example-prompted GPT-J model (ensemble).}
\end{table*}

==> old/sections/4_experiment.tex <==
\subsection{Experiments Setup}

\paragraph{Dataset Details}
- Few-shot splits? 

\paragraph{Knowledge Distillation}
For \textsc{ChEMU-Ref}, we randomly sample 1000 paragraphs from the chemical patent corpus collected in \citet{bai-etal-2021-pre} to generate pseudo labels, and select the most confident 500 or 1000 predictions to train a smaller student model. For \textsc{Recipe-Ref}, we use the Recipe1M+ dataset \citep{Marn2019Recipe1MAD} as the source of unlabeled data, and perform the same knowledge distillation procedure as we do it for \textsc{ChEMU-Ref}.

\paragraph{Evaluation Metrics}
- Lenient F1 
- Strict Accuracy 

\paragraph{Implementation Details} 
- Foundational Model GPT-J-6B and GPT-3/J1-Jumbo for ARRAU
- Tune hyperparameters on dev set?
- Number of prompts per prediction
- Truncation strategies
- Number of examples in the prompt: fix 2-shot.

\subsection{Baseline Models}

\paragraph{Pipeline Neural Models}
- Recent-X baseline 
- Random baseline

\paragraph{Joint Neural Models}
- Fang et al 
- Yu et al 

\paragraph{Extractive QA Finetuning}

\paragraph{Text Generation Finetuning} GPT2, T5, T0, etc. 

\begin{table}[!h]
\centering
\scalebox{0.95}{
\begin{tabular}{lcccccc}
\toprule
% \textbf{Datasets} & \multicolumn{6}{c}{\textbf{CheEMU-Ref}} & \multicolumn{6}{c}{\textbf{RecipeRef}} & \multicolumn{4}{c}{\textbf{ARRAU}}\\
% \cmidrule(l{5pt}r{5pt}){2-7} \cmidrule(l{5pt}r{5pt}){8-13} \cmidrule(l{5pt}r{5pt}){14-17} 
\multirow{2}{*}{\textbf{Model}} & \multicolumn{6}{c}{$|\Dc_{train}|$} \\
\cmidrule(l{5pt}r{5pt}){2-7}
 & \textit{4} & \textit{8} & \textit{16} & \textit{32} & \textit{64} & \textit{full} \\
\hline
\textsc{Recent-5} & & & & &\\
\textsc{Recent-all} & & & & &\\
\textsc{Random} & & & & &\\
\textsc{Fang et al. 2021} & & & &  & &\\
% \textsc{Yu et al. 2021} & & & &  & &\\
\hline
\textsc{GPT2-XL} & &  & &\\
\textsc{T5-3B} & &&  & &\\
\textsc{T0-3B} & & &  & &\\
\hline 
\textsc{SingleRandom} & & & & & &\\
\textsc{SingleSimilar} & & & & &\\
\textsc{Mixture} & & & & &\\
\bottomrule
\end{tabular}
}
\caption{Our main results on the test set. For each size of $K$ (\textit{i.e.} $|\mathcal{D}_{train}|$) (column), we report the mean and standard deviation across 5 different training set samples.}
\label{tab:main}
\end{table}

\subsection{Results}

- Main results: Table \ref{tab:main}
- Main results: Figure \ref{fig:f1_vs_k}

\begin{figure}[!t]
    \centering
    \includegraphics[scale=0.50]{figures/single.pdf}
    \caption{Results on applying in-context learning on few-shot split antecedent. Naively applying in-context learning did not perform better than an existing baseline method. However, oracle result shows there exists prompts that significantly outperforms the baseline, even approaching fully supervised methods (purple line). This suggests ample room for improvements.
    \Max{This figure can also be a table-- whichever demonstrates the point and tells the story better. Also some curves are placeholders}}
    \label{fig:ensemble_motivation}
\end{figure}

\begin{table}[!t]
\centering
\begin{tabular}{lcccc}
\hline
 & \textbf{$k$=32} & \textbf{$k$=64} & \textbf{$k$=full} \\
\hline
Best Baseline & & & \\
\hline
Best Single Model & & & \\
- Span-based Verbalizer & \\
\hline
Best Combined Model & \\
- Span-based Verbalizer & \\
\hline
\end{tabular}
\caption{We ablate single and combined models for selected values of $k$
\Max{I am a hesitant on what the columns should be. If we use $k$, should we also report $k$=full?}}
\label{tab:calibration}
\end{table}

\paragraph{Results} We applied standard in-context learning approaches to our problem. For prompt retrieval methods, we experimented with random retrieval and KNN retrieval, where we rank all the training examples using an off-the-shelf retrieval methods, given a test example. For prompt ordering, we experimented with having the most-to-least and least-to-most similar orderings. Figure \ref{fig:ensemble_motivation} plots the F1 score vs. the size of $\mathcal{D}_{train}$. We observe that while similarity-based retrieval does fare better than random retrieval, all in-context learning models (SingleRandom, SingleMostSimilarForward, SingleMostSimilarBackward) do not improve over the baseline result (Baseline). In addition, there is no distinct difference between two prompt ordering strategies, which is in-line with conclusions from previous work \cite{Lu2022Fantastically, liu2021makes}. 

Interestingly, the oracle model shows that there exists optimal prompt that significantly outperforms the baseline and even approaches the fully supervised setting. This shows promises for developing effective in-context learning methods for split-antecedent resolution.



==> old/sections/5_analysis.tex <==
\subsection{In-context Behaviors}

\begin{figure}[!t]
    \centering
    \includegraphics[scale=0.50]{figures/numPrompts_vs_f1.pdf}
    \caption{\ar{TODO: remove similarity-based methods.  This is the main thing that jumps out from the figure, but I think the difference is due to similarity methods effectively having access to fewer training examples, so it's hard to explain in the paper.  I think the main point we want to make here is that there is a huge and consistent performance improvement as more prompts are added.} We plot the F1 score vs. the number of prompts ensemble, which also corresponds to the efficiency of our approach (measured in floating-point operations). The more prompts in the ensemble, the longer the inference time will take. We can see that the more prompts the better; but the performance plateaued between 100 - 200 prompts. \Max{Other unit for this can be GPU hours}}
    \label{fig:numPrompts_vs_f1}
\end{figure}

\paragraph{Number of prompts vs. Performance} Figure \ref{fig:f1_vs_promptNUM} TODO conclusion

\subsection{Quantitative/Error Analysis}

==> old/sections/6_related.tex <==
\paragraph{Split-antecedent Resolution} \Max{Goal here is to motivate the task}

\paragraph{In-context Learning} \Max{Goal here is to motivate approach}
Orthogonally, we can apply recently developed techniques to find the best perfomant prompt for a single model \cite{Lu2022Fantastically, Zhao2021Calibrate}. In our work, we found that simple ensemble procedures described already achieve significant gains comparing to existing baselines. We hypothesize that applying and extending these techniques to our task can further strengthen the results, which we leave for future investigations. \maxle{This paragraph/justification is conditioned on whether we want to try out their approaches. If we do, replace description with new description. If we don't, can we make this justification stronger?}

\paragraph{Few-shot Learning} \Max{Goal here is to motivate approach}
- Prompting 
- Also works that study the phenomenon of LMs
Besides training larger LMs on bigger datasets or dataset of tasks (T0, that other work from Google), notable research directions in this area include formulating problems or objectives that close the gap between finetuning and pretraining tasks , and/or building around the phenomenon of \textit{in-context learning}, popularized by GPT-3 \cite{liu2021makes, Rubin2021LearningTR, metaICL, XieICLasBayesianInference}. Most of these work are evaluated on popular text classification and question-answering benchmarks (cite some benchmarks), leaving out other challenging NLP tasks (TODO example of such tasks?)
